Diversity Analysis of Bit-Interleaved Coded Multiple Beamforming

In this paper, diversity analysis of bit-interleaved coded multiple beamforming (BICMB) is extended to the case of general spatial interleavers, removing a condition on their previously known design criteria and quantifying the resulting diversity order. The diversity order is determined by a parameter Qmax which is inherited from the convolutional code and the spatial de-multiplexer used in BICMB. We introduce a method to find this parameter by employing a transfer function approach as in finding the weight spectrum of a convolutional code. By using this method, several Qmax values are shown and verified to be identical with the results from a computer search. The diversity analysis and the method to find the parameter are supported by simulation results. By using the Singleton bound, we also show that Qmax is lower bounded by the product of the number of streams and the code rate of an encoder. The design rule of the spatial de-multiplexer for a given convolutional code is proposed to meet the condition on the maximum achievable diversity order.

==> deleted.tex <==


In Fig. \ref{fig:4x4}, the BER curve of $1/4$-rate convolutional
code in $S=4$ case is in parallel with that of $1/2$-rate code in
$S=2$ case at the BER range between $10^{-5}$ and $10^{-7}$, which
are a little steeper than the $4 \times 4$ OSTBC code. They have
$Q_{max} = 1$ from the Table \ref{tab:alpha_vectors}. However, the
other curves with legends of $S=4$ $R=1/3$, $S=3$ $R=1/2$ and $S=4$
$R=1/2$, whose $Q_{max}=2$, are almost in parallel with that of $3
\times 3$ OSTBC code at the same BER range. Therefore, the slopes of
$S=4$ $R=1/4$ and $S=2$ $R=1/2$ approach to $16$ while the slopes of
the other three curves approach to $9$ at high SNR.


\hline \hline
\multirow{3}*{$4$} & $1/4$ & $4$ & $3$ & & $1$ \\
\cline{2-6}
& $1/3$ & $12$ & $12$ & $[0\, 4\, 5\, 3]$ $[0\, 4\, 8\, 6]$ & $2$ \\
\cline{2-6}
& $1/2$ & $4$ & $6$ & $[0\, 1\, 2\, 2]$ $[0\, 2\, 2\, 2]$ & $2$ \\


\\
&+ Z^8(a^4 b^4 + a^5 b^2 c + a^4 b^3 c + a^3 b^4 c + a^2 b^5 c +\\
&\quad a^5 b c^2 + 7 a^4 b^2 c^2 + 12 a^3 b^3 c^2 + 7 a^2 b^4 c^2
+\\
&\quad a b^5 c^2 + a^4 b c^3 + 12 a^3 b^2 c^3 + 12 a^2 b^3 c^3 +\\
&\quad a b^4 c^3 + a^4 c^4 + a^3 b c^4 + 7 a^2 b^2 c^4 + a b^3 c^4
+\\
&\quad b^4 c^4 + a^2 b c^5 + a b^2 c^5)


From (\ref{eq:d_order}), we can see that BICMB achieves the full
diversity order $MN$ if $Q_{max}$ equals to $1$. Compared to the
previously introduced criteria in \cite{akayTC06BICMB}, this
condition relaxes the requirement for the full diversity order.

The combination of the ML bit metrics of (\ref{eq:ML_bit_metrics})
and $\mathbf{\tilde{U}}$ detector at the receiver is not the unique
solution to get the optimum BER performance. Appropriate bit metrics
corresponding to a linear detector, such as zero-forcing (ZF) or
minimum mean square error (MMSE) detector, were shown to be
equivalent to the bit metrics of (\ref{eq:ML_bit_metrics}) with
$\mathbf{\tilde{U}}$ detector \cite{ErsinTCOMM08}.


==> presentation.tex <==
\begin{align}
P\left(\mathbf{c} \rightarrow \mathbf{\hat{c}}\right) &=
E\left[P\left(\mathbf{c} \rightarrow \mathbf{\hat{c}}|
\mathbf{H} \right)\right] \nonumber \\
& \leq E \left[ \frac{1}{2} \exp \left(- \frac{d^2_{min}
\sum\limits_{s=1}^{S} \alpha_{s} \lambda_{s}^2}{4 N_0} \right)
\right]
\end{align}

\begin{displaymath}
\begin{array}{ll}
d_{min} & \textrm{the minimum Euclidean distance in the constellation} \\
\alpha_s & \textrm{the number of times the $s^{th}$ subchannel is used}\\
&\textrm{corresponding to $d_H$ bits under consideration,} \\
&\textrm{satisfying } \sum_{s=1}^{S} \alpha_s = d_H\\
\lambda_s & \textrm{singular value of the $s^{th}$ subchannel}\\
N_0 & \textrm{variance of Gaussian noise channel}
\end{array}
\end{displaymath}

\begin{align}
\sum_{s=1}^{S} \alpha_{s} \lambda_{s}^2 \geq \alpha_{nzmin}
\sum_{k=1,\alpha_k > 0}^{S} \lambda_{k}^2
\end{align}

\begin{displaymath}
\begin{array}{ll}
\alpha_{nzmin} & \textrm{the minimum among non-zero elements in $\alpha$-vector}\\
\end{array}
\end{displaymath}

\begin{align}
P\left(\mathbf{c} \rightarrow \mathbf{\hat{c}}\right) &=
E\left[P\left(\mathbf{c} \rightarrow \mathbf{\hat{c}}|
\mathbf{H} \right)\right] \nonumber \\
& \leq E \left[ \frac{1}{2} \exp \left(- \frac{d^2_{min}
\sum\limits_{s=1}^{S} \alpha_{s} \lambda_{s}^2}{4 N_0} \right)
\right] \\
& \leq E \left[ \frac{1}{2} \exp \left(- W \sum\limits_{k=1}^{K}
\mu_{\ell{(k)}} \right) \right]
\end{align}

\begin{displaymath}
\begin{array}{ll}
W = & \frac{d^2_{min} \alpha_{nzmin}}{4 N_0} = \frac{d^2_{min} \alpha_{nzmin}}{4 N} SNR \\
K & \textrm{the number of non-zero $\alpha$'s}\\
\ell(k) &\textrm{an index to indicate the $k^{th}$ non-zero $\alpha$} \\
\mu_s = & \lambda_s^2
\end{array}
\end{displaymath}

\begin{align}
\rho \left(\mu_1, \cdots, \mu_N \right) = \prod^N_{i=1}
\mu_{i}^{M-N} \prod^N_{j>i} \left (\mu_i - \mu_j \right )^2
e^{-\sum\limits_{i=1}^N \mu_i}
\end{align}

\begin{align}
\hat{\rho} \left(\mu_1, \cdots, \mu_N \right) = \prod^N_{i=1}
\mu_{i}^{M-N} \prod^N_{j>i} \left (\mu_i - \mu_j \right )^2
e^{-\left( \mu_1 + \sum\limits_{i=1}^K \mu_{\ell(i)}\right)}
\end{align}

\begin{align}
\hat{f} \left( \mu_{\ell(1)}, \cdots, \mu_{\ell(K)} \right ) &=
\int_0^{\infty} \int_0^{\mu_1} \cdots \int_0^{\mu_{\ell(1)-2}}
\int_0^{\mu_{\ell(1)}} \cdots \int_0^{\mu_{N-1}}
\hat{\rho} \left(\mu_1, \cdots, \mu_N \right) \\
&\qquad\qquad\qquad\qquad\qquad\qquad\times d_{\mu_N} \cdots
d_{\mu_{\ell(1)+1}} d_{\mu_{\ell(1)-1}}
\cdots d_{\mu_2} d_{\mu_1} \\
&= r \left( \mu_{\ell(1)}, \cdots, \mu_{\ell(K)} \right)
e^{-\sum\limits_{i=1}^K \mu_{\ell(i)}}
\end{align}

\begin{align}
P\left(\mathbf{c} \rightarrow \mathbf{\hat{c}}\right) &\leq \eta
\left( \frac{d_{min}^2 \alpha_{nzmin}}{4N} SNR
\right)^{-(M-Q+1)(N-Q+1)} \label{eq:PEP_result}
\end{align}

\begin{displaymath}
\begin{array}{ll}
g(\cdot) & \textrm{PEP corresponding to each error event} \\
W_I(d) & \textrm{the total input weight of error events at Hamming
distance $d$}\\
\end{array}
\end{displaymath}

\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
$S$ & rate & $d_{free}$ & dominant $\alpha$-vectors & $Q_{max}$ \\
\hline \hline
\multirow{3}*{$2$} & $1/2$ & $10$ & $[3\,\, 7]$ $[4\,\, 6]$ $[5\,\, 5]$ & $1$ \\
\cline{2-5}
& $2/3$ & $6$ & $[0\,\, 12]$ $[0\,\, 14]$ $[0\,\, 15]$ & $2$ \\
\cline{2-5}
& $3/4$ & $5$ & $[0\,\, 8]$ $[0\,\, 10]$ $[0\,\, 12]$ & $2$ \\
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
$S$ & rate & $d_{free}$ & dominant $\alpha$-vectors & $Q_{max}$ \\
\hline \hline
\multirow{4}*{$3$} & $1/3$ & $15$ & $[3\,\, 6\,\, 6]$ $[5\,\, 4\,\, 6]$ $[4\,\, 6\,\, 6]$ & $1$ \\
\cline{2-5}
& $1/2$ & $10$ & $[0\,\, 7\,\, 7]$ $[0\,\, 8\,\, 6]$ $[0\,\, 9\,\, 7]$ & $2$ \\
\cline{2-5}
& $2/3$ & $6$ & $[0\,\, 4\,\, 5]$ $[0\,\, 6\,\, 3]$ $[0\,\, 4\,\, 6]$ & $2$ \\
\cline{2-5}
& $3/4$ & $5$ & $[0\,\, 0\,\, 13]$ $[0\,\, 0\,\, 15]$ $[0\,\, 0\,\, 17]$& $3$ \\
\hline
\end{tabular}
\end{center}
\end{table}

